Improving Multi-Task Generalization via Regularizing Spurious Correlation

Multi-Task Learning (MTL) is a powerful learning paradigm to improve generalization performance via knowledge sharing. However, existing studies find that MTL could sometimes hurt generalization, especially when two tasks are less correlated. One possible reason that hurts generalization is spurious correlation, i.e., some knowledge is spurious and not causally related to task labels, but the model could mistakenly utilize them and thus fail when such correlation changes. In MTL setup, there exist several unique challenges of spurious correlation. First, the risk of having non-causal knowledge is higher, as the shared MTL model needs to encode all knowledge from different tasks, and causal knowledge for one task could be potentially spurious to the other. Second, the confounder between task labels brings in a different type of spurious correlation to MTL. We theoretically prove that MTL is more prone to taking non-causal knowledge from other tasks than single-task learning, and thus generalize worse. To solve this problem, we propose Multi-Task Causal Representation Learning framework, aiming to represent multi-task knowledge via disentangled neural modules, and learn which module is causally related to each task via MTL-specific invariant regularization. Experiments show that it could enhance MTL model's performance by 5.5% on average over Multi-MNIST, MovieLens, Taskonomy, CityScape, and NYUv2, via alleviating spurious correlation problem.

==> sections/related_old_.tex <==
% \section{Related Works}

% \subsection{Optimization for MTL}

% Most studies to improve multi-task learning are model-agnostic. A very common observation is that during optimization, different tasks might conflict with each other, leading to conflicting gradients and compete the model capacity. As a result, some dominating tasks will take a large portion of gradient updates, and thus even the average loss seems to reduce, some dominated tasks are actually perform quite bad.

% To tackle such problem, researchers develop different optimization tricks. 
% Here I present three lines of work: 1) loss weighting; 2) gradient modulation; 3) knowledge distillation; 4) task scheduling.


% \subsection{Loss Weighting}
% During optimization, some tasks will be under-estimated. A naive way is to weight the loss of each task, and increase the weights for those bad-performing (or uncertain) tasks.
% There are many works that learn this weight on-the-fly, with different criteria:

% \paragraph{Uncertainty}
% \citet{DBLP:conf/cvpr/KendallGC18} treat the
% multi-task network as a probabilistic model, and derive a weighted multi-task loss function by maximizing the likelihood
% of the ground truth output. For each task, it models the model output as a Gaussian distribution $\mathcal{N}(f_i(x), \sigma_i^2)$, where $\frac{1}{\sigma}$ could be interpreted as the uncertainty for this task, which could be learned and control the weight for each task.


% There are many works try to balance loss weights by how fast a task converge. For example, \citet{DBLP:conf/cvpr/LiuJD19} proposes the ratio of current loss to previous loss. 
% Several other works propose similar loss-ratio based weighting.
% \citet{DBLP:conf/icml/ChenBLR18} optimize the loss weights so that the weighted average of gradients is close to each gradient.

% \subsection{Task Relationship Learning}
% Similar to task weighting, learning task relationship will find the similar tasks to train together (by assigning higher weights to data / task), or have higher parameter sharing.

% \cite{DBLP:conf/icml/StandleyZCGMS20} conducts an empirical study on the tasonomy dataset \citep{DBLP:conf/cvpr/ZamirSSGMS18}. The authors find several interesting observations: First, there were mixed results on whether or not multi-task training improved over the single-task baselines, with many multi-task networks performing worse than the single-task counterparts (negative transfer). Next, the performance gain from single-task to multi-task training varies wildly with the training setting, implying that the effectiveness of MTL is not as dependent on the relationship of the tasks themselves as we might have once thought. Surprisingly, the study also finds no correlation between the multi-task affinity and the transfer affinity between tasks, which again shows that there are many more factors behind joint task learning dynamics (in both multi-task and transfer learning) than just the nature of the tasks in consideration.

% Starting from Taxonomy\citep{DBLP:conf/cvpr/ZamirSSGMS18}, a series of work try to mine task similarity to help transfer learning / multi-task learning. Taxonomy first train a task-specific encoder, and see how well another task's decoder perform using source task's encoder. In this way, they can compute task similarity, and use Boolean Interger Programming problem to get a sparse taxonomy graph.

% Though effective, such method takes a lot of combination trial. Recently, \cite{DBLP:conf/bmvc/VandenhendeGGB20} train single model on each task, and compare the representation distribution (such as Representation Similarity Analysis (RSA)), and \cite{DBLP:conf/nips/SongCWSS19} use attribution map to calculate task similarity.

% Also, there are several works try to construct task embedding by a pre-trained network, which can be used to infer task similarity to novel tasks


% \subsection{Gradient Modulation}

% One major challenge of MTL optimization is that multiple tasks might have conflicting gradients, i.e., $cos(G_i, G_j) < 0$. To directly tackle this problem, a series of works manipulate the gradients.



% \cite{DBLP:conf/nips/Lopez-PazR17} introduces Gradient Episodic Memory (GEM) for continual learning, a problem formulation in which a model learns multiple tasks sequentially, instead of simultaneously as in MTL. GEM keeps an episodic memory of training examples from past learned tasks, and enforces the following constraint at each update step $t$ when training on task $i$.
% If the condition cannot be fulfilled, then $G_i(t)$ is replaced by $\hat(G)_i(t)$.
% Solving such optimization problem is time-consuming. Thus, a later work A-GEM relax the condition to the average of gradients. 
% This is exactly what introduced in PCGrad, though introduced in a different problem setup. This paper randomly select a pair of gradients and project one to the other if gradient contradict. 
% GradVac\citep{DBLP:conf/iclr/WangTF021} propose to learn adaptive cosine value between each pair of task to maintain those negative task pair (doing so cannot avoid gradient conflict, but just try to keep mutual task relationship fix).
% GradDrop\citep{DBLP:conf/nips/ChenNHLKCA20} randomly drop part of the gradient if they conflict. The final algorithm is similar to PCGrad. 


% % \subsection{Covariate Shift}
% % \cite{DBLP:conf/iclr/0002ZR20} finds that even if the decision function is similar (or even the same), the data / representation distribution's co-variance matters a lot to information transfer in multi-task learning, so they add a alignment layer to match the distribution.
